ACOUSTIC-TURF: Acoustic-based Privacy-Preserving COVID-19 Contact Tracing

In this paper, we propose a new privacy-preserving, automated contact tracing system, ACOUSTIC-TURF, to fight COVID-19 using acoustic signals sent from ubiquitous mobile devices. At a high level, ACOUSTIC-TURF adaptively broadcasts inaudible ultrasonic signals with randomly generated IDs in the vicinity. Simultaneously, the system receives other ultrasonic signals sent from nearby (e.g., 6 feet) users. In such a system, individual user IDs are not disclosed to others and the system can accurately detect encounters in physical proximity with 6-foot granularity. We have implemented a prototype of ACOUSTIC-TURF on Android and evaluated its performance in terms of acoustic-signal-based encounter detection accuracy and power consumption at different ranges and under various occlusion scenarios. Experimental results show that ACOUSTIC-TURF can detect multiple contacts within a 6-foot range for mobile phones placed in pockets and outside pockets. Furthermore, our acoustic-signal-based system achieves greater precision than wireless-signal-based approaches when contact tracing is performed through walls. ACOUSTIC-TURF correctly determines that people on opposite sides of a wall are not in contact with one another, whereas the Bluetooth-based approaches detect nonexistent contacts among them.

==> math_definition.tex <==
%%% load AMS-Latex Package
\usepackage{amssymb}
\usepackage{amsmath,amsfonts}
% \usepackage{amsthm}
\usepackage{amsopn}
\usepackage{bm} % bold symbol
\usepackage{multirow}

% define vector and matrix symbols
\newcommand{\vct}[1]{\boldsymbol{#1}} % vector
\newcommand{\mat}[1]{\boldsymbol{#1}} % matrix
\newcommand{\cst}[1]{\mathsf{#1}}  % constant

%%%% Special math symbols
\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\R}{\field{R}} % real domain
% \newcommand{\C}{\field{C}} % complex domain
\newcommand{\F}{\field{F}} % functional domain
\newcommand{\I}{\field{I}} % functional domain
\newcommand{\T}{^{\textrm T}} % transpose


%% operator in linear algebra, functional analysis
\newcommand{\inner}[2]{#1\cdot #2}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\twonorm}[1]{\left\|#1\right\|_2^2}
\newcommand{\onenorm}[1]{\|#1\|_1}
\newcommand{\Map}[1]{\mathcal{#1}}  % operator in functions, maps such as M: domain1 --> domain 2

% operator in probability: expectation, covariance, 
\newcommand{\ProbOpr}[1]{\mathbb{#1}}
% independence
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\ind}[2]{{#1} \independent{#2}}
\newcommand{\cind}[3]{{#1} \independent{#2}\,|\,#3} % conditional independence
\newcommand{\expect}[2]{%
\ifthenelse{\equal{#2}{}}{\ProbOpr{E}_{#1}}
{\ifthenelse{\equal{#1}{}}{\ProbOpr{E}\left[#2\right]}{\ProbOpr{E}_{#1}\left[#2\right]}}} % Expectation: syntax: E{1}{2} = E_1[2], E{}{2}=E[2], E{1}{} = E_1
\newcommand{\var}[2]{%
\ifthenelse{\equal{#2}{}}{\ProbOpr{VAR}_{#1}}
{\ifthenelse{\equal{#1}{}}{\ProbOpr{VAR}\left[#2\right]}{\ProbOpr{VAR}_{#1}\left[#2\right]}}} % Expectation: syntax: V{1}{2} = V_1[2], V{}{2}=V[2], V{1}{} = V_1
\newcommand{\cndexp}[2]{\ProbOpr{E}\,[ #1\,|\,#2\,]}  % conditional expectation

% operator in optimization
\DeclareMathOperator{\argmax}{arg\,max}
\DeclareMathOperator{\argmin}{arg\,min}
\DeclareMathOperator{\softmax}{softmax}

% special functions
\newcommand{\trace}[1]{\operatornamewithlimits{tr}\left\{#1\right\}}
\newcommand{\diag}{\operatornamewithlimits{diag}}
\newcommand{\sign}{\operatornamewithlimits{sign}}
\newcommand{\const}{\operatornamewithlimits{const}}

% special display
\newcommand{\parde}[2]{\frac{\partial #1}{\partial  #2}}


% environment
% \newtheorem{thm}{Theorem}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{proposition}[theorem]{Proposition}

% shorthand
\newcommand{\vtheta}{\vct{\theta}}
\newcommand{\vmu}{\vct{\mu}}
\newcommand{\vc}{\vct{c}}
\newcommand{\vp}{\vct{p}}
\newcommand{\vq}{\vct{q}}
\newcommand{\vx}{{\vct{x}}}
\newcommand{\vy}{\vct{y}}
\newcommand{\vz}{{\vct{z}}}
\newcommand{\vu}{\vct{u}}
\newcommand{\vo}{{\vct{o}}}
\newcommand{\va}{\vct{a}}
\newcommand{\vb}{\vct{b}}
\newcommand{\vr}{\vct{r}}
\newcommand{\vt}{\vct{t}}
%\newcommand{\vpsi}{\vct{\psi}}
% \newcommand{\vs}{\vct{s}}
% \newcommand{\vv}{\vct{v}}
\newcommand{\vw}{\vct{w}}
\newcommand{\vbeta}{\vct{\beta}}
\newcommand{\vgamma}{\vct{\gamma}}
\newcommand{\vzero}{\vct{0}}
\newcommand{\vf}{\vct{f}}
\newcommand{\vh}{\vct{h}}
\newcommand{\vg}{\vct{g}}
\newcommand{\vphi}{\vct{\phi}}
\newcommand{\vpsi}{\vct{\psi}}
\newcommand{\ones}{\vct{1}}
\newcommand{\mU}{\mat{U}}
\newcommand{\mA}{\mat{A}}
\newcommand{\mB}{\mat{B}}
\newcommand{\mD}{\mat{D}}
\newcommand{\mW}{\mat{W}}
\newcommand{\mH}{\mat{H}}
\newcommand{\mS}{\mat{S}}
\newcommand{\mJ}{\mat{J}}
\newcommand{\mM}{\mat{M}}
\newcommand{\mT}{\mat{T}}
\newcommand{\mZ}{\mat{Z}}
\newcommand{\mO}{\mat{O}}
\newcommand{\mY}{\mat{Y}}
\newcommand{\mL}{\mat{L}}
\newcommand{\mI}{\mat{I}}
\newcommand{\mK}{\mat{K}}
\newcommand{\mSigma}{\mat{\Sigma}}
\newcommand{\mOmega}{\mat{\Omega}}
\newcommand{\cC}{\cst{C}}
\newcommand{\cM}{\cst{M}}
\newcommand{\cN}{\cst{N}}
\newcommand{\cQ}{\cst{Q}}
\newcommand{\cD}{\cst{D}}
\newcommand{\cL}{\cst{L}}
\newcommand{\cK}{\cst{K}}
\newcommand{\cH}{\cst{H}}
\newcommand{\cR}{\cst{R}}
\newcommand{\cU}{\cst{U}}
\newcommand{\cS}{\cst{S}}
\newcommand{\sQ}{\mathcal{Q}}
\newcommand{\sS}{\mathcal{S}}
\newcommand{\sF}{\mathcal{F}}
\newcommand{\sC}{\mathcal{C}}


% 
\newcommand{\nx}{\tilde{x}}
\newcommand{\vnx}{{\tilde{\vx}}}
\newcommand{\vnz}{{\tilde{\vz}}}
%\newcommand{\deltavx}{(\vnx-\vx)}
\newcommand{\deltavx}{\delta_\vx}
\newcommand{\vmx}{\bar{\vx}}
\newcommand{\vmz}{\bar{\vz}}
\newcommand{\sigmax}{\mSigma_{\vx}}
\newcommand{\sigmaz}{\mSigma_{\vz}}
\newcommand{\no}{\tilde{o}}
\newcommand{\vno}{{\tilde{\vo}}}
\newcommand{\nell}{\tilde{\ell}}
\newcommand{\jacob}{\mat{J}}
\newcommand{\hess}{\mat{H}}
\newcommand{\mloss}{\hat{\ell}}

%
\newcommand{\eat}[1]{}
\newcommand{\method}[1]{\textsc{#1}}
% \newcommand{\task}[1]{\textbf{#1}}
\newcommand{\GDC}{\method{GDC}\xspace}
\newcommand{\SDN}{\method{SDN}\xspace}
\newcommand{\GSTD}{\method{GS3D}\xspace}
\newcommand{\vPIXOR}{\method{PIXOR$^\star$}\xspace}
\newcommand{\PIXOR}{\method{PIXOR}\xspace}
\newcommand{\PRCNN}{\method{P-RCNN}\xspace}
\newcommand{\SRCNN}{\method{S-RCNN}\xspace}
\newcommand{\PL}{\method{pseudo-LiDAR}\xspace}
\newcommand{\AVOD}{\method{AVOD}\xspace}
\newcommand{\Frustum}{\method{F-PointNet}\xspace}
\newcommand{\Mono}{\method{Mono3D}\xspace}
\newcommand{\DOP}{\method{3DOP}\xspace}
\newcommand{\DORN}{\method{DORN}\xspace}
\newcommand{\MLF}{\method{MLF}\xspace}
\newcommand{\MLFmono}{\method{MLF-mono}\xspace}
\newcommand{\MLFstereo}{\method{MLF-stereo}\xspace}

\newcommand{\APBEV}{AP$_\text{BEV}$\xspace}
\newcommand{\AP}{AP$_\text{3D}$\xspace}

\newcommand{\PSMNet}{\method{PSMNet}\xspace}
\newcommand{\PSMNetpd}{\method{PSMNet}\xspace}
\newcommand{\DispNet}{\method{DispNet}\xspace}
\newcommand{\DispNetS}{\method{DispNet-S}\xspace}
\newcommand{\DispNetC}{\method{DispNet-C}\xspace}
\newcommand{\SPSstereo}{\method{SPS-stereo}\xspace}
\newcommand{\PnP}{\method{PnP}\xspace}


\def\mathbi#1{\textbf{\em #1}}

==> paper/7.related.tex <==
%!TEX root=..\new-paper.tex


We discuss related work in two regards: (1) the recent efforts on coronavirus tracing; (2) acoustic MAC.\@

\subsection{Mobile Phone Based Pandemic Tracking}
There are multiple competing technologies toward pandemic tracking by mobile devices.

Recently, researchers have proposed several approaches for tracing the spread of the coronavirus among people using pervasive mobile phones.

Covid Watch~\cite{CovidWatch} uses Bluetooth signals to detect when users are in proximity to each other and alerts them anonymously if
they were in contact with someone later confirmed to have COVID-19.
The system does so without anyone—including the government—being able
to track who exposed whom. The services provided by Covid Watch
include Bluetooth contact tracing, GPS heatmaps, and user
recommendations.

Similarly, PACT~\cite{PACT} uses inter-phone Bluetooth
communications (including energy measurements) as a proxy for
inter-person distance measurement. Through applied cryptography, this
system can collect and maintain weeks of contact events. Later, PACT
augments these events with infection notifications leading to exposure
notifications to all mobile phone owners who have had
medically-significant contact (in terms of distance and time) with
infected people in the past medically-significant time period (e.g.,
two weeks).

Singapore launched the TraceTogether~\cite{TraceTogether} mobile
application (app) to boost COVID-19 contact tracing efforts. By
downloading the app and consenting to participate in it, TraceTogether
allows users to ``proactively help'' in the contact tracing process,
according to a joint press release~\cite{tracetogether2}. The app
works by exchanging short distance Bluetooth signals between phones to
detect other app users who are in close proximity. Current Ministry of
Health (MOH) guidelines define close proximity as between two and five
meters apart for 30 minutes.

Apple and Google~\cite{googleandapple} recently announced that they are
working together for the first time on a protocol that will alert
users if they have been exposed to the coronavirus. Their joint effort
enables the use of Bluetooth technology to help governments and health
agencies reduce the spread of the virus, with user privacy and
security central to the design.


As Table~\ref{tab:compare_tracing} shows, we propose A-Turf, an
alternative method of contact tracing using acoustic signals due to
their privacy-preserving nature---specifically, no unique MAC address
disclosure and limited communication range---which is exactly what we
need in order to avoid privacy concerns and false positives (e.g.,
reported contacts between faraway users). Bluetooth based solutions
may use mechanisms such as randomization to avoid unique MAC address
disclosure. However, it is very difficult for them to limit Bluetooth
communication range within physical proximity (such as a 6-foot range).
Further, our acoustic solution can be enhanced to capture
finer-grained contact tracing such as face orientation,
handshakes, and conversations.

\subsection{Acoustic communication}
Several works related to acoustic sensing use machine learning-based techniques for audio sensing tasks. For example, DeepEar~\cite{lane2015deepear} focused on multiple place identification such as restaurants, bars, coffee and ice-cream shops. 


\begin{table}[htb]
  \centering
  \begin{tabular}{p{2cm}p{3cm}p{3cm}p{2cm}p{3.5cm}}\hline
  \textbf{Approach}  & \textbf{Number of Devices} & \textbf{Relative Motion Support} & \textbf{Distance (m)} & \textbf{Device Position} \\\hline
    Hush~\cite{novak2018ultrasound} & 2 & No & $< 0.5$ & On obstacle\\\hline
    U-Wear~\cite{santagati2015u} & $> 2$ & No & $< 0.5$ & On body (fixed)\\\hline
    Dhwani~\cite{nandakumar2013dhwani} & 2 & No & $< 0.2$\footnotemark & No obstacles\\\hline
    DopEnc~\cite{zhang2017acoustic} & 1--3 & No & 1--1.5 & N/A \\\hline
    A-Turf & Up to 10 & Yes & 2 & Any position, occluded \\\hline
  \end{tabular}
  \vspace*{1mm}
  \caption{Comparison of Multi-Access Communications Approaches}%
  \label{tab:compare_mac}
\end{table}
\footnotetext{Dhwani's short distance is for security reasons.}

As stated before, multiple nearby contacts are possible among nearby
people carrying mobile phones. Acoustic signal retransmission among
the phones is necessary because collisions are unavoidable. Rapidly
sending and receiving acoustic signals amidst all phones poses a
non-trivial challenge. There has been much research on acoustic signal
communication and networking. Here, we just focus on scenarios with
multiple phones.


As illustrated in Table~\ref{tab:compare_mac}, there is a body of work that
enables acoustic communications between devices that are equipped with
microphones and speakers. Novak et al. presented Hush~\cite{novak2018ultrasound}, a software
modem that utilizes very high frequency sound to send data between
commodity smart mobile devices. Hush performs fast modulation
unobtrusively among users and achieves a low error rate. The system
incorporates a fingerprinting scheme that hinders masquerades by
attackers by allowing the receiver to learn and recognize packets sent
from the intended sender. However, the communication distance spans
only 5--20\,cm, which is not feasible for accurate contact tracing.
U-Wear~\cite{santagati2015u} enables data dissemination between ultrasonic wearable
devices. Dhwani~\cite{nandakumar2013dhwani} employs audible sound for near field
communications between smartphones using OFDM and FSK modulations.
This work focuses on high data rate and throughput for communications.
DopEnc~\cite{zhang2017acoustic} can automatically identify persons with whom users interact and considers coordinating multiple access in
order to measure the Doppler effect.

In summary, no existing work has addressed the scenario where there
are multiple moving users (up to 10) within a 2-meter range, occluded
from each other, and whose mobile phones are in pockets or purses. We
design A-Turf to address this scenario.




